GShard: Scaling Giant Models with Conditional Computation and Automatic Sharding

Neural network scaling has been critical for improving the model quality in many real-world machine learning applications with vast amounts of training data and compute. Although this trend of scaling is affirmed to be a sure-fire approach for better model quality, there are challenges on the path such as the computation cost, ease of programming, and efficient implementation on parallel devices. GShard is a module composed of a set of lightweight annotation APIs and an extension to the XLA compiler. It provides an elegant way to express a wide range of parallel computation patterns with minimal changes to the existing model code. GShard enabled us to scale up multilingual neural machine translation Transformer model with Sparsely-Gated Mixture-of-Experts beyond 600 billion parameters using automatic sharding. We demonstrate that such a giant model can efficiently be trained on 2048 TPU v3 accelerators in 4 days to achieve far superior quality for translation from 100 languages to English compared to the prior art.

==> backup.tex <==
We enumerate approaches for scaling sync training. Switching to async training regime has quality implications, and thus limits usable model architectures. 


\begin{description}
    \item[Dense scaling] Generic, with no constraints on model architecture.
    \begin{itemize}
        \item Linear scaling with model and batch size \Q{FLOPS = \#weights * batch\_size}
        %%%
        \item Wide vs Deep
        \begin{itemize}
            \item Machine Translation
            \item Images
        \end{itemize}
        %%%
        \item Breaking single core memory limits efficiently: Pipelining / GPipe
        \begin{itemize}
            \item Mixes layer-by-layer model parallelism and data parallelism with multiple replicas
            \item irreducible bubble
        \end{itemize}
    \end{itemize}
    %%%
    \item[Sparse scaling] Conditional computation is key for sublinear scaling with number of model weights (Noam, 17)
    \begin{itemize}
        \item MoE RNN (Noam, 17)
        \item MoE Transformer
        \begin{itemize}
            \item Mixes fully model parallel MoE layer and fully data parallel Attention and generic FeedForward layers
            \item Our (noam@, ylc@) previous work mesh\_tensorflow. SPMD. Language on top of TensorFlow with explicit named Tensor dimensions that enables defines sharding, and a subset of ops with translation to generic TensorFlow ops. (Python API, Compiles into TensorFlow).
        \end{itemize}
    \end{itemize}
\end{description}

Difficulties:
\begin{itemize}
\item Graph partitioning lacks efficiency (aka gpipe bubble / dense computation).
\item Mesh requires re-implementing ops and rewriting the programs.
\end{itemize}

